Recursive fragmentation of a polarized quark

The thesis is devoted to the study of the fragmentation process of polarized quarks, and in particular of the Collins effect used for the extraction of the quark transversity distribution. The aim is to include the spin degree of freedom in the hadronization part of Monte Carlo event generators by using the string+${}^3P_0$ model. The model is reviewed here and the relevant functions have been written in a form suitable for a Monte Carlo implementation. Two main variants of the model for pseudoscalar meson production are formulated and both of them have been implemented in stand alone Monte Carlo programs. After tuning one single parameter, the simulation results are compared with the measured Collins and dihadron transverse spin asymmetries showing a satisfactory qualitative agreement. Given this encouraging outcome, one of them has been interfaced with the hadronization part of the PYTHIA event generator. The quark transversity distribution has been implemented in the generator allowing to simulate for the first time the polarized SIDIS process. The comparison of the simulated transverse spin asymmetries with the experimental data is found to be very promising. As final development, vector meson production and decays have been included in a consistent way with the rules of quantum mechanics. The effect of vector meson production on transverse spin asymmetries has been studied in detail with a stand alone Monte Carlo program showing that the new model is a promising and powerful model for the description of the polarized quark fragmentation process.

==> Chapters/Chapter5_preliminary.tex <==
\chapter{Vector meson production in polarized quark fragmentation}
In the previous chapters the fragmentation process of polarized quarks was restricted to the production of pseudoscalar mesons and the comparison of the MC simulations with the experimental data gave already a satisfactory agreement.
However, in order to have a more quantitative description of the experimental data, the species of hadron types that can be produced in the fragmentation process has to be extended.

The introduction of vector mesons changes the basic features of the fragmentation process as for instance the rank structure of the hadrons produced directly in the string fragmentation (\textit{primary hadrons}). Due to their strong decays they affect the kinematical distributions of the final observable hadrons, which now are a mixture of primary hadrons and of \textit{secondary hadrons}, i.e. those produced in the decays of primary vector mesons.
Due to the larger combinatorics, the effect is expected to be more important when looking at hadron pairs in the same jet. For instance, restricting to first and second rank hadrons, from a $u$ quark jet we can produce a $\pi^+\pi^-$ pair only through the channel $u\rightarrow \pi^+ + d\rightarrow \pi^+\pi^- + u$. Instead, after the introduction of vector mesons, the channels $u\rightarrow \rho^0+u\rightarrow \pi^+\pi^- + \pi^+ + d$ or $u\rightarrow \rho^+ + d\rightarrow \pi^+\pi^0+\pi^-+d$ and many others open up.
In this case there are 17 different channels to produce the charged pion pair whereas there is only one channel for the direct production of the pair.

In addition, vector mesons carry spin information that is transferred to the angular distribution of the decay products in the decay process. This changes also the propagation of the quark polarization along the fragmentation chain with respect to M19.
 
%The fragmentation process of a quark in a hadron pair is also important for the extraction of the quark transversity distribution. 
 
 
 
 
ONGOING WRITING
 
 

 \section{The new string+${}^3P_0$ model}
 \subsection{Splitting matrix for vector meson production}
 The splitting matrix for vector meson production, can be derived by the analogue expression for pseudoscalar meson production given in Eq. (\ref{eq: T final}) with the following observations.
 
 The coupling matrix of quarks to pseudoscalar mesons introduced in Eq. (\ref{eq:coupling ps}) has to be replaced by the coupling of quarks to a vector meson which is \cite{DS09}
 \begin{eqnarray}\label{eq: Gamma vm}
\nonumber     \Gamma_{h,V} &=& G_T\,\boldsymbol{\sigma}\T\sigma_z\cdot \textbf{V}\T^* + G_L\, 1_{2\times 2}\,V_z^*\\
     &=&\Gamma_{h,\alpha}V_\alpha^*.
 \end{eqnarray}
$\textbf{V}^*$ is the polarization vector of the vector meson expressed in the vector meson rest frame normalized such that $\textbf{V}^*\cdot\textbf{V}=1$. It is obtained boosting the corresponding polarization four-vector expressed in the string rest frame by a sequence of two boosts. A longitudinal boost $\Lambda_L^{-1}(p_z)$ which brings to the frame where the vector meson has vanishing longitudinal momentum, and a transverse boost $\Lambda_T^{-1}(\pt)$ opposite to the direction of the vector meson transverse momentum. This particular composition of Lorentz boosts brings to the vector meson rest frame and respects the LR symmetry requirement \cite{DS09}. $G_L$ and $G_T$ are two complex constants for the coupling to a vector meson with longitudinal and transverse linear polarization. The label $\alpha$ can be $\rm{L}$ or $\rm{T}$.


Since vector mesons are resonances it is necessary to introduce a mass spectrum. This can be done by rewriting the phase space factor for a stable particle as
\begin{eqnarray}\label{eq:phase space stable hadron}
\nonumber       \frac{dZ}{Z}d^2\pt &=& \frac{dp^+}{p^+}d^2\pt\\
\nonumber        &=& dp^+dp^- 2\delta(p^2-m_h^2)d^2\pt.
\end{eqnarray}
For a stable particle with mass $m_h^2$, the delta function ensures that the hadron momentum satisfies the mass-shell condition $p^2=m_h^2$. To take into account the finite width of a resonance, such function is replaced by a complex spectral function $D_h(p^2)$ such that $|D_h(p^2)|^2$ is the resonance mass distribution. We take it as the relativistic Breit-Wigner distribution
\begin{equation}\label{eq:BW distribution}
    D_h^{(i)}(p^2)=\frac{\sqrt{m_h\gamma_{h}^{(i)}/\pi}}{p^2-m_h^2+i\,m_h\gamma_{h}}.
\end{equation}
We have indicated with $\gamma_{h}^{(i)}$ the partial width for the $i$-th channel. The total width is then $\gamma_{h}=\sum_i \gamma_h^{(i)}$. The factor $\gamma_h^{(i)}/\gamma_h$ is the branching ratio corresponding to the $i$-th channel. The branching ratio and the meson mass $m_h$ are taken from PDG.
Moreover the mass distribution is normalized such that
\begin{equation}
    \int_{-\infty}^{+\infty} \sum_i |D_h^{(i)}(p^2)| dp^2 = 1.
\end{equation}

With these considerations the phase space factor in Eq. (\ref{eq:phase space stable hadron}) becomes
\begin{eqnarray}\label{eq:phase space vm}
\nonumber \frac{dZ}{Z}d^2\pt &\rightarrow& dp^+dp^-d^2\pt |D_h^{(i)}(p^2)|^2\\
&=&dp^2\frac{dZ}{Z}d^2\pt |D_h^{(i)}(p^2)|^2,
\end{eqnarray}
where we have traded $p^-$ for $p^2$ using the relation $dp^+dp^-=dp^2dp^+/p^+$.


Taking into account the coupling matrix in Eq. (\ref{eq: Gamma vm}) and the modification of the phase space factor in Eq. (\ref{eq:phase space vm}), the analogue of the splitting matrix in Eq. (\ref{eq: T final}) for vector meson emission is
\begin{eqnarray}\label{eq: T final vm}
\nonumber    T_{q',h,q}&=& T_{q',h,q}^{(\alpha)}V_{\alpha}^*\\
\nonumber &=& C_{q',h,q}\,\check{g}(\varepsilon_h^2)\left[(1-Z/\varepsilon_h^2\right]^{a/2}\,\exp{\left[-\bl\varepsilon_h^2/(2Z)\right]}\\
    &\times& \Delta_{q'}(\kpt)\Gamma_{h,V}\hat{u}_q^{-1/2}(\kt).
\end{eqnarray}
The factor $C_{q',h,q}$ implements the splitting in flavor space. It takes into account the suppression of $s$ quarks with respect to $u$ and $d$ quarks and weights coming from the isospin wave function. Contrary to the pseudoscalar case, there is no suppression among the flavor diagonal states, i.e. the $\omega$ meson is not suppressed with respect to the $\rho^0$ meson.
Furthermore, for a vector meson the transverse energy is $\varepsilon_h^2=p^2+\ptpt$.

For vector meson production, the corresponding reduced single quark density matrix $\hat{u}_q$ introduced in Eq. (\ref{eq: hat uq}) becomes
\begin{eqnarray}\label{eq: hat uq vm}
 \nonumber   \hat{u}_q(\kt) &=&\sum_{h}\,|C_{q',h,q}|^2\int dp^2\,|D_h(p^2)|^2\, \int dZZ^{-1} d^2\kpt\,\left(\frac{1-Z}{\varepsilon_h^2}\right)^a\,e^{-\bl\varepsilon_h^2/Z}\,\check{g}^2(\varepsilon_h^2)\\
    &\times& \sum_{\alpha}\Gamma^{\dagger}_{h,\alpha}\Delta^{\dagger}_{q'}(\kpt)\Delta_{q'}(\kpt)\Gamma_{h,\alpha}
    \end{eqnarray}.


\subsection{Splitting function for vector meson production}
For the calculation of the splitting function for vector meson production, we make again the choice $C_1$ for the function $\check{g}$ as introduced in Eq. (\ref{eq:choice-c1}). The corresponding $\hat{u}_q(\kt)$ matrix obtained from Eq. (\ref{eq: hat uq vm}) is then
\begin{equation}
    \hat{u}_q= \textbf{1}\,(2|G_T|^2+|G_L|^2)\,\sum_h |C_{q',h,q}|^2 \left(|\mu|^2+\langle \ktkt\rangle_{f\T}\right),
\end{equation}
where the weighting operation is introduced in Eq. (\ref{eq:weight fT}). Hence also in this case the $\hat{u}_q$ matrix is proportional to the unit matrix and as a consequence the intermediate spin density matrix $\hat{\rho}_{int}(q)$ coincides with the true spin density matrix $\rho(q)$ of $q$.
Also, the splitting $q\rightarrow h + q'$ in flavor space is described by the coefficient $C_{q',h,q}$ as in Eq. (\ref{eq:p_q->h simple 3P0}).

Using the splitting matrix in Eq. (\ref{eq: T final vm}) and Eq. (\ref{eq:choice-c1}), the splitting function for vector meson production is
\begin{eqnarray}\label{eq:F_explicit vm}
\nonumber F_{q',h,q}(p^2,Z,\pt;\kt,\textbf{S}_q)&=& \frac{|C_{q',h,q}|^2}{\sum_H |C_{q',H,q}|^2}\,|D_h(p^2)|^2\, \left(\frac{1-Z}{\varepsilon_h^2}\right)^a \frac{\exp{(-\bl \varepsilon_h^2/Z)}}{N_a(\varepsilon_h^2)} \\
\nonumber &\times& \frac{|\mu|^2+\kptkpt}{|\mu|^2+\langle \ktkt\rangle_{f\T}} f_{\T}^2(\kptkpt) \\
&\times& \left[ 1+\frac{|G_L|^2}{2|G_T|^2+|G_L|^2}\frac{2\IM(\mu)\,\rm{k'}_{\rm{T}}}{|\mu|^2+\kptkpt}\textbf{S}_{q}\cdot\tilde{\textbf{n}}(\kpt) \right].
\end{eqnarray}
As we can notice, the last line of the splitting function is a source of a global Collins effect for the vector meson. It is related to the Collins analysing analysing power for a rank one pseudoscalar particle through the equation
\begin{equation}\label{eq: ap vm / ap ps}
    \frac{a^{q_A\uparrow\rightarrow VM+X}|_{r=1}}{a^{q_A\uparrow\rightarrow PS+X}|_{r=1}} = - \frac{|G_L|^2}{2|G_T|^2+|G_L|^2},
\end{equation}
namely the global Collins effect for a leading vector meson is opposite to the Collins effect for a leading pseudoscalar. It is also scaled by the factor $1/(1+2|G_T|/|G_L|)$ which for $|G_L|=|G_T|$ gives the Czyzewski prediction \cite{Czyzewski-vm}, i.e. the ratio between the the Collins analysing power for a leading vector meson and that of a leading pseudoscalar is $-1/3$. This value, however, follows from the non relativistic quark model and need not be necessarily satisfied. In general, the factor $|G_L|/|G_T|$ can be different from unity.

For a deeper investigation of the relation in Eq. (\ref{eq: ap vm / ap ps}, it is useful to decompose the splitting function for vector meson emission in Eq. (\ref{eq:F_explicit vm}) as
\begin{eqnarray}
F_{q',h,q}(p^2,Z,\pt;\kt,\textbf{S}_q)=\sum_V F_{q',h,q}^{(V)}(p^2,Z,\pt;\kt,\textbf{S}_q)
\end{eqnarray}
where $V=\rm{M},\rm{N},\rm{L}$ and the linear polarization states $\rm{\textbf{M}}$, $\rm{\textbf{N}}$ and $\rm{\textbf{L}}$ have already been introduced in Eq. (\ref{eq: MNL states}).
Hence $F_{q',h,q}^{V}$ indicates the splitting function for the emission of a vector meson with linear polarization given by $V$.

Carrying out explicitly the calculations, it is
\begin{eqnarray}
\label{eq: F vm M} F_{q',h,q}^{(M)}(p^2,Z,\pt;\kt,\textbf{S}_q)&=& \dots \left[ |G_T|^2+|G_T|^2\frac{2\IM(\mu)\,\rm{k'}_{\rm{T}}}{|\mu|^2+\kptkpt}\textbf{S}_{q}\cdot\tilde{\textbf{n}}(\kpt) \right] \\
\label{eq: F vm N} F_{q',h,q}^{(N)}(p^2,Z,\pt;\kt,\textbf{S}_q)&=& \dots \left[ |G_T|^2-|G_T|^2\frac{2\IM(\mu)\,\rm{k'}_{\rm{T}}}{|\mu|^2+\kptkpt}\textbf{S}_{q}\cdot\tilde{\textbf{n}}(\kpt) \right] \\
\label{eq: F vm L} F_{q',h,q}^{(L)}(p^2,Z,\pt;\kt,\textbf{S}_q)&=& \dots \left[ |G_L|^2+|G_L|^2\frac{2\IM(\mu)\,\rm{k'}_{\rm{T}}}{|\mu|^2+\kptkpt}\textbf{S}_{q}\cdot\tilde{\textbf{n}}(\kpt) \right]
\end{eqnarray}
where the dots represent the first and second lines of Eq. (\ref{eq:F_explicit vm}) and are the same in all three cases.  From these equations it is clear that the Collins effect for vector mesons longitudinally polarized along $\textbf{L}$ and transversely polarized along $\textbf{M}$ is opposite to that of pseudoscalar mesons. Whereas, vector mesons transversely polarized along $\rm{\textbf{N}}$ have the same Collins effect as pseudoscalar mesons. If the polarization of the vector meson is not analyzed, i.e. is summed over, we get then the relation in Eq. (\ref{eq: ap vm / ap ps}).

Finally, looking at Eq. (\ref{eq:F_explicit vm}), we note also that for the generation of a vector meson in simulations, it is more convenient to generate first the splitting in flavor space, then the mass of the vector meson according to the spectral function $|D_h(p^2)|^2$, afterwards $\kpt$ and eventually $Z$.

\subsection{The spin correlations between $h$ and $q'$}
ONGOING WRITING...



\subsection*{Joint spin density matrix of $q'$ and $h$}

\subsection*{Spin density matrix of the vector meson}

\subsection*{Polarization of the quark $q'$}


\subsection{The decay process of a polarized vector meson}

\subsection*{Two body decay}


\subsection*{Three body decay}

\subsection*{Acceptance density matrix}



%\section{Positivity conditions}





\section{Monte Carlo implementation}



\section{Results from simulations}
In the present section, we show some results as obtained from simulations with the model M20. The introduction of vector mesons requires the addition of four new parameters. Two of them concern the probabilities that a particular $q\bar{q}'$ pair be a vector meson relative to the probability for the same pair to be a pseudoscalar. In particular $\left(f_{VM}/f_{PS}\right)_{ud}=0.68$ for a non-strange $q\bar{q}'$ pair and $\left(f_{VM}/f_{PS}\right)=0.725$ if at least one quark of the pair is a strange quark. These values are the same as the standard values in PYTHIA 8.

The other two concern are the ratio $|G_L|/|G_T|$, related to the probabilities that a quark couples to a vector meson with longitudinal or transverse linear polarizations, and the relative phase $\theta_{LT}$ between $G_L$ and $G_T$ which allows vector mesons to possess oblique linear polarization in the $(\xu,\zu)$ plane.
We take as initial values $|G_L|=|G_T|$ and $\theta_{LT}=0$. This produces a ratio between the Collins analysing power of a first rank $\rho$-meson and the corresponding first rank pion of $-1/3$ \cite{Czyzewski-vm}.
However, the sensibility of the observables to the values of these parameters is investigated.

The results that will be shown below are obtained from simulations of transversely and fully polarized $u$ quarks which initial energy is obtained using the same sample of $x_B$ and $Q^2$ values used also in the simulations with M18 and M19. The primordial transverse momentum is initially switched off.


\subsection{Kinematical distributions, analysing power and sensitivity to free parameters}
The relations between the $Z$ and $\ptpt$ distributions of vector mesons with different ranks are the same as those for the pseudo-scalar analogues as shown in Chapter 4 for M19 and therefore will not be repeated here. In particular the $Z$ distribution of a first rank vector meson is pushed to a somewhat lower $Z$ values with respect to the $Z$ distributions for larger ranks, as in Fig. \ref{fig:Z distribution}.


More interesting, is the comparison between the kinematical distributions of vector mesons and the primary pseudo-scalar mesons. As standard cuts for the kinematical distributions we require $p_{\rm{T}}>0.1\,\rm{GeV}$ when looking at the $z_h$ distribution and in addition also $z_h>0.2$ when looking at the $\ptpt$ distributions. Figure \ref{fig:zh pT prim pi+ vs rho+} shows the comparison between the $z_h$ (left panel) and $\ptpt$ (right panel) distributions for primary $\pi^+$ (dotted histogram) and $\rho^+$ mesons (continous histogram). The corresponding comparison for $\pi^-$ and $\rho^-$ is shown in Fig. \ref{fig:zh pT prim pi- vs rho-}. We can notice that the vector mesons carry typically larger fractions of the initial quark energy, due to their larger mass with respect to the corresponding pseudo-scalar configuration. Indeed, we recall that the hadron mass enters in the exponential of the longitudinal splitting function, as can be seen from Eq. (\ref{eq:F_explicit vm}). We notice also differences in the $\ptpt$ distributions of vector and pseudo-scalar meson. In particular, vector mesons have typically smaller transverse momenta than pseudoscalar mesons, as expected from the classical string+${}^3P_0$ model shown in Fig. Indeed, the transverse momenta of the quark that constitue the vector meson are on the average directed along opposite directions whereas in the pseudoscalar case they lay along the same direction. The same features are seen both for positively and negatively charged mesons.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi+prim_vs_rho+.pdf}
  \end{minipage}
  \caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^+$ (dotted histogram) and for $\rho^+$ (continuous histogram).}\label{fig:zh pT prim pi+ vs rho+}
\end{figure}
\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
	\includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi-prim_vs_rho-.pdf}
\end{minipage}
\caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^-$ (dotted histogram) and for $\rho^-$ (continuous histogram).}\label{fig:zh pT prim pi- vs rho-}
\end{figure}

It is instructive to compare also the kinematical distributions between vector mesons and their decay products. For instance, in Fig. \ref{fig:zh pT rho+ vs pi+ from rho+} we compare the $z_h$ and $\ptpt$ distributions of $\rho^+$ mesons (continous histogram) with the corresponding distributions of positive pions produced in the $\rho^+$ decay. It is clear that the decay pions have typically smaller fractional energies with respect to the parent $\rho^+$ meson. Concerning the $\ptpt$ distributions we notice that the decay pions have slightly smaller transverse momenta compared to those of their parent vector mesons. The tranverse momentum of a decay pion receives two contributions: it inherits part of the parent $\rho^+$ meson and it receives a transverse kick in the decay process, with respect to the $\rho^+$ line of flight. An approximate relation between the average transverse momentum of the decay pion $\langle \pt^2\rangle_{\pi^+}$, the transverse momentum $\langle \pt^2\rangle_{\rho^+}$ of the $\rho^+$ and the transverse momentum $\langle \pt^2\rangle_{\pi^+/\rho^+}$ that the $\pi^+$ receives in the decay process is $\langle \pt^2\rangle_{\pi^+}\simeq (z_{\pi^+}/z_{\rho^+})^2\langle \pt^2\rangle_{\rho^+}+\langle \pt^2\rangle_{\pi^+/\rho^+}$.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi+decay_vs_rho+.pdf}
  \end{minipage}
  \caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for $\rho^+$ (continous histogram) and for $\pi^+$ produced in the decay of $\rho^+$ mesons (dotted histogram).}\label{fig:zh pT rho+ vs pi+ from rho+}
\end{figure}
\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
	\includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi-decay_vs_rho-.pdf}
\end{minipage}
\caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for $\rho^-$ (continous histogram) and for $\pi^-$ produced in the decay of $\rho^+$ mesons (dotted histogram).}\label{fig:zh pT rho- vs pi- from rho-}
\end{figure}


The effect of the $\rho^+$ decay on the $z_h$ and $\ptpt$ distributions of primary positive pions is studied in Fig. \ref{fig:zh pT prim pi+ vs pi+ from rho+}. The dotted histogram represents the distribution of primary pions whereas the continous one represents the distribution of primary and decay pions. The analogue distributions for $\pi^-$ and $\rho^-$ are shown instead in Fig. \ref{fig:zh pT prim pi- vs pi- from rho-}. In both cases we notice that pions produced in the decay of vector mesons enhance the $z_h$ and the $\ptpt$ distributions mostly at small values of fractional energies and transverse momenta, as expected from Figs. \ref{fig:zh pT rho- vs pi- from rho-}-\ref{fig:zh pT rho- vs pi- from rho-}.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi+prim_vs_pi+rho+decay.pdf}
  \end{minipage}
  \caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^+$ (dotted histogram), for $\pi^+$ from the decay of $\rho^+$ mesons (continous thin histogram) and for the sum of the two contributions (continous thick histogram).}\label{fig:zh pT prim pi+ vs pi+ from rho+}
\end{figure}
\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
	\includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi-prim_vs_pi-rho-decay.pdf}
\end{minipage}
\caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^-$ (dotted histogram), for $\pi^-$ produced in the decay of $\rho^-$ mesons (continous thin histogram) and for the sum of the two contributions (continous thick histogram).}\label{fig:zh pT prim pi- vs pi- from rho-}
\end{figure}

Figure \ref{fig:pi+ from rho / prim. pi+} shows the ratio as function of $z_h$ and of $p_{\rm{T}}$ between secondary charged pions coming from the decays of $\rho^{\pm}$ and $\rho^0$ mesons and the primary ones. Circles represent positive pions whereas triangles represent negative pions.
Again, the effect of $\rho$ meson decay increases with decreasing $z_h$. Already at $z_h\simeq 0.7$ half of positive pions are secondary pions and the ratio tends to one at small fractional energies. At very large $z_h$ the contamination from secondary pions decreases fast, especially for negative pions. The contamination to the $\pi^-$ sample from secondary mesons has a different shape with respect to $\pi^+$ due to the different $z_h$ distributions of primary $\pi^+$ and primary $\pi^-$ present in $u$ quark jets.
Also, as function of $p\T$ the contamination from secondary mesons is large at small transverse momenta and vanishes with increasing $p\T$. The contamination at small $p\T$ is larger for negative pions because primary $\pi^-$ can be produced from second rank and are typically characterized by larger transverse momenta with respect to rank one. On the other hand, secondary $\pi^-$ can be produced from primary $\rho^0$ which have small transverse momenta.


\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/fraction_pions_rho.pdf}
  \end{minipage}
  \caption{Ratio between positive pions (circles) and negative pions (triangles) produced in decays of $\rho^{\pm,0}$ mesons and primary positive and negative pions, as function of $z_h$ (left panel) and as function of $p_{\rm{T}}$ (right plot).}\label{fig:pi+ from rho / prim. pi+}
\end{figure}

TO BE ADDED: TABLE WITH FRACTIONS OF $\pi$, $\rho$, $\omega$, $\phi$ ETC IN THE JETS...

Including the decays of all vector mesons, the $z_h$ and $\ptpt$ distributions of final pions are enhanced at least by a factor of two with respect to the primary pions. The contribution of secondary pions is visible for $z_h\leq 0.8$ and for $\ptpt\leq 1.0\, \rm{GeV^2}$, as can be seen in Fig. \ref{fig:zh pT prim pi+ vs all pi+} for positive pions and in Fig. \ref{fig:zh pT prim pi- vs all pi-} for negative pions.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi+prim_vs_pi+tot.pdf}
  \end{minipage}
  \caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^+$ (dotted histogram), secondary pions (continous thin histogram) and both primary and secondary $\pi^+$ (continuous thick histogram) when decays of all vector mesons are considered.}\label{fig:zh pT prim pi+ vs all pi+}
\end{figure}
\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
	\includegraphics[width=1.0\linewidth]{./FiguresVM/kinematics/pi-prim_vs_pi-tot.pdf}
\end{minipage}
\caption{Distributions of $z_h$ (left panel) and of $\ptpt$ (right panel) for primary $\pi^-$ (dotted histogram), secondary pions (continous thin histogram) and both primary and secondary $\pi^-$ (continuous thick histogram) when decays of all vector mesons are considered.}\label{fig:zh pT prim pi- vs all pi-}
\end{figure}



\subsection*{Collins analysing power}
We have already anticipated that leading vector mesons have opposite Collins analysing power with respect to leading pions. This can be deduced comparing the splitting function for vector meson production in Eq. (\ref{eq:F_explicit vm}) with the corresponding splitting function for pseudoscalar meson emission of M19 given in Eq. (\ref{eq:F_explicit simple 3P0}).

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/collins_rho.pdf}
  \end{minipage}
  \caption{Collins analysing power for $\rho^+$ (squares), $\rho^0$ (triangles) and $\rho^-$ (circles) as function of $z_h$ (left panel) and as function of $p\T$ (right panel).}\label{fig:collins for rho}
\end{figure}

This can be seen more clearly in Fig. \ref{fig:collins for rho} which shows the Collins analysing power for $\rho$ mesons as function of $z_h$ (left panel) and as function of $p\T$ (right panel).
All $\rho$ mesons have positive analysing power, therefore with opposite sign with respect to that of the leading pions in M19 as expected from the classical string+${}^3P_0$ mechanism applied to the case of vector meson production. Indeed, $\rho^+$ and $\rho^0$ mesons are produced already at first rank which is characterized by a positive analysing power and this fixes the sign of the rank-integrated analysing power. Instead, $\rho^-$ mesons are produced from second rank either with negative analysing power after a first rank vector meson or with positive analysing power after a first rank pseudoscalar meson. Considering the suppression of light $q\bar{q}'$ states with respect to the analogue pseudo-scalar states, the latter case is favoured. Hence the analysing power of $\rho^-$ mesons is also positive.

More interesting is the effect of the introduction of vector mesons on the Collins analysing power for observable hadrons like pions and kaons, which are a mixture of directly produced mesons (primary mesons) and those coming from the decay of primary vector mesons (secondary mesons).
Vector mesons have a twofold contribution, namely they affect both the Collins analysing power of primary pseudoscalar mesons and contribute to the overall Collins effect of observable pseudoscalar mesons due to their strong decays.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/confronto_M19_M20_pioni_diretti.pdf}
  \end{minipage}
  \caption{Comparison between the Collins analysing power as function of $z_h$ (left panel) and as function of $p\T$ (right panel) for positive (circles) and negative (triangle) pions as obtained with M18 (open markers) and as obtained with M20 (full markers) with vector meson decay switched off.}\label{fig:collins pions M19 vs M20}
\end{figure}

The effect of vector meson production on the primary charge pions is shown in Fig. \ref{fig:collins pions M19 vs M20}. It compares the Collins analysing power for $\pi^+$ (circles) and $\pi^-$ (triangles) as obtained without vector mesons as in the model M19 (open markers) and after introducing vector meson production with their decays switched off (full markers). We notice that the Collins effect for positive pions is slightly larger in M20 than in M19  slightly whereas for negative pions the holds the reverse.
This can be understood as follows. As in M19, in M20 positive pions are produced as first rank with negative analysing power. As second rank they are produced either after a first rank pseodoscalar meson, hence with negative analysing power as in M19, but also after a first rank vector meson, hence with positive analysing power like the first rank. The latter contribution enhances slightly the overall analysing power. The slight reduction of the analysing power for negative pions, is understood by the same considerations. They are produced from rank two with opposite analysing power depending whether the first rank meson is a vector or a pseudoscalar state.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/collins_pions_from_rho+.pdf}
  \end{minipage}
  \caption{Comparison between the Collins analysing power as function of $z_h$ (left panel) and as function of $p\T$ (right panel) for $\rho^+$ positive (squares) and the analysing power of the decay $\pi^+$ (circles) and $\pi^0$ (triangles).}\label{fig:collins rho+ vs decay pi+ pi0}
\end{figure}

In the decay process, the global Collins effect of vector mesons is transferred to the decay products and this is shown in Fig. \ref{fig:collins rho+ vs decay pi+ pi0} for $\rho^+$ (rectangles) and the decay $\pi^+$ (circles) and $\pi^0$ (triangles). First, we notice that both as function of $z_h$ (left panel) and as function of $p\T$ (right panel), the decay pions have the same analysing power, since the decay process is invariant under parity. Instead, compared to the analysing power of the parent $\rho^+$, that of the decay pions is somewhat different.

The requirement of decay pions with large $z_h$, selects preferably $\rho^+$ mesons with longitudinal linear polarization which have exactly the opposite Collins effect with respect to the leading pions, as can be seen from Eq. (\ref{eq: F vm L}). Instead, the Collins analysing power of $\rho^+$ shown is summed over the $\rho^+$ polarizations. Hence, the decay pions at large $z_h$ come from a $\rho^+$ that has a larger analysing power with respect to what can be seen in the left plot of Fig. \ref{fig:collins rho+ vs decay pi+ pi0}.
The differences on the analysing power at large transverse momenta can be understood with similar considerations. Decay pions with large transverse momenta, come most likely from $\rho^+$ mesons also with large transverse momenta. From the classical string+${}^3P_0$ picture, it can be seen that a $\rho^+$ with a large transverse momentum can be produced at second or higher rank when the transverse momenta of the constituent quarks are aligned along the same direction. This happens if the meson is polarized along the $\textbf{N}$ axis, namely along the normal to its production plane. In this case, from Eq. (\ref{eq: F vm N}), we see that the $\rho^+$ has exactly the same Collins effect as a pseudoscalar meson, which for rank two is positive. This explains the larger analysing power of $\pi^+$ and of $\pi^0$ at large transverse momenta.
The negative sign of the analysing power of decay pions at small transverse momenta, can be understood looking at Fig. Pions emitted almost at $90^{\deg}$ in the $\rho^+$ rest frame, have very different tranverse momenta in the string rest frame. In the configuration of Fig., the $\rho^+$ is produced with $0<\phi_{\rho}<\pi/2$ whereas one of the two decay pions is produced with small transverse momentum with respect to the string axis and with azimuthal angle in the range $-3\pi/2<\phi_{\pi}<0$, hence with opposite analysing power with respect to the $\rho^+$.
The same features are seen also in the decay of $\rho^-$ and $\rho^0$ mesons.


\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_rhop_pioni.pdf}
  \end{minipage}
  \caption{Effect of $\rho^+$ decay on the Collins analysing power of final positive (circles) and negative (triangle) pions. The open markers represent primary pions when the decays of vector mesons are switched off whereas the closed markers when switching on the $\rho^+$ decay.}\label{fig:effetto rhop pioni}
\end{figure}
The effect of $\rho^+$ decay on the Collins analysing power of charged pions is shown in Fig. \ref{fig:effetto rhop pioni}. The open markers represent primary pions when vector meson decays are inhibited whereas closed markers represent the case when only $\rho^+$ decay is switched on. As expected, the $\pi^+$ analysing power is reduced and the reduction can be clearly seen as function of $z_h$ and of $p\T$. It is interesting to notice that now the analysing power as function of $z_h$ for $\pi^+$ is bent and does not retain the linear trend typical of primary pions. The effect of $\rho^+$ decay is large as function of $p\T$, especially for $p\T<1\,\rm{GeV}$ as expected from Fig. \ref{fig:pi+ from rho / prim. pi+}.

The decay of $\rho^-$ mesons have a similar effect on the $\pi^-$ analysing power. In this case, however, the effect is smaller since negative pions produced in the decay of $\rho^-$ mesons are characterized by an analysing power of the same sign as primary negative pions. More interesting is the decay of $\rho^0$ mesons which affects both positive and negative pions, as can be seen in Fig. \ref{fig:effetto rhoz pioni}.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_rhoz_pioni.pdf}
  \end{minipage}
  \caption{Effect of $\rho^0$ decay on the Collins analysing power of final positive (circles) and negative (triangle) pions. The open markers represent primary pions when the decays of vector mesons are switched off whereas the closed markers when switching on the $\rho^0$ decay.}\label{fig:effetto rhoz pioni}
\end{figure}

Switching on the decays of all $\rho$ mesons we get the result shown in Fig. \ref{fig:effetto rho pioni}. Again, open markers show the analysing power of primary charged pions whereas closed markers show the analysing power of primary and secondary pions. The effect is large for both charges and as function of both $z_h$ and $p\T$. The effect is stronger in the case of positive pions, which secondary sub-sample has analysing power with opposite sign with respect to the primary one.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_rho_pioni.pdf}
  \end{minipage}
  \caption{Effect of $\rho$ mesons decay on the Collins analysing power of final positive (circles) and negative (triangle) pions. The open markers represent primary pions when the decays of vector mesons are switched off whereas the closed markers when switching on the $\rho$ mesons decay.}\label{fig:effetto rho pioni}
\end{figure}

Switching on $\omega$ and $\phi$ decays does not change sensibly further the Collins analysing power of charged pions. Neither do the decays of strange vector mesons. Hence the final plot switching on all vector meson decays is shown in Fig. \ref{fig:effetto all vm pioni}. The main effect on the analysing power of primary pions is produced by the decays of $\rho$ mesons.

Without going through the same analysis also for kaons, for which hold the same considerations as for pions, we report just the total effect of all vector meson decays on the Collins analysing power for charged kaons. It is shown in Fig. \ref{fig:effetto all vm kaons} as function of $z_h$ (left panel) and as function of $p\T$ (right panel) for $K^+$ (circles) and $K^-$ (triangles). The open markers show the analysing power for primary charged kaons when the decays of all vector mesons are switched off, whereas the full markers the corresponding analysing power for primary and secondary kaons when all vector meson decays are switched on. In this case, the effect of vector meson decay is larger for $K^+$. The mesons $K^{*+}$ and $K^{*0}$ provide the larger contribution.

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_allvm_pioni.pdf}
  \end{minipage}
  \caption{Effect of vector mesons decay on the Collins analysing power of final positive (circles) and negative (triangle) pions. The open markers represent primary pions when the decays of vector mesons are switched off whereas the closed markers when switching on all vector mesons decay.}\label{fig:effetto all vm pioni}
\end{figure}

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_strangeVM_kaons.pdf}
  \end{minipage}
  \caption{Effect of vector mesons decay on the Collins analysing power of final positive (circles) and negative (triangle) kaons. The open markers represent primary kaons when the decays of vector mesons are switched off whereas the closed markers when switching on all vector mesons decay.}\label{fig:effetto all vm kaons}
\end{figure}

%\subsection{Sensibility to the free parameters}
In the previous plots we assumed $|G_L|=|G_T|$ and $\theta_{LT}=0$. It is instructive to study how sensible are the final observable results to variations of these parameters.
In Fig. \ref{fig:effetto G collins ap} is shown the effect of variations of $|G_L|/|G_T|$ on the Collins analysing power of positive (full markers) and negative (open markers) pions. Triangles are obtained for $|G_L|=0.2|G_T|$, circles for $|G_L|=|G_T|$ and squares for $|G_L|=5|G_T|$. The first choice favors the coupling of quarks to vector mesons with transverse linear polarization. The second one gives an equal weight to longitudinal and transverse linear polarizations. The third favors the coupling to vector mesons with longitudinal linear polarization. Decays are switched on for all species of vector mesons. From the left panel of Fig. \ref{fig:effetto G collins ap} we notice that the effect of varying $|G_L|/|G_T|$ can be seen mostly for positive pions with $z_h>0.6$ or with $p\T<0.5\,\rm{GeV}$.

%When the coupling to vector mesons with longitudinal linear polarization is favored.....

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_G_collins.pdf}
  \end{minipage}
  \caption{Effect of $|G_L|/|G_T|$ on the Collins analysing power for charged pions when the decays of all vector mesons are switched on. Triangles are obtained for $|G_L|/|G_T|=0.2$, circles for $|G_L|=|G_T|$ and squares for $|G_L|=5|G_T|$. }\label{fig:effetto G collins ap}
\end{figure}



\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_theta_collins.pdf}
  \end{minipage}
  \caption{Effect of $\theta_{LT}$ on the Collins analysing power for charged pions obtained from simulations when the decays of all vector mesons are switched on and $|G_L|/|G_T|=1$. Triangles are obtained for $\theta_{LT}=-\pi/2$, circles for $\theta_{LT}=0$ and squares for $\theta_{LT}=\pi/2$. }\label{fig:effetto theta collins ap with GL = GT}
\end{figure}

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_theta_collins_G02.pdf}
  \end{minipage}
  \caption{Effect of $\theta_{LT}$ on the Collins analysing power for charged pions obtained from simulations when the decays of all vector mesons are switched on and $|G_L|/|G_T|=5$. Triangles are obtained for $\theta_{LT}=-\pi/2$, circles for $\theta_{LT}=0$ and squares for $\theta_{LT}=\pi/2$. }\label{fig:effetto theta collins ap with GL = 5 GT}
\end{figure}

\begin{figure}[tb]
\centering
\begin{minipage}[t]{.6\textwidth}
  \includegraphics[width=1.0\linewidth]{./FiguresVM/collins/effetto_theta_collins_G5.pdf}
  \end{minipage}
  \caption{Effect of $\theta_{LT}$ on the Collins analysing power for charged pions obtained from simulations when the decays of all vector mesons are switched on and $|G_L|/|G_T|=0.2$. Triangles are obtained for $\theta_{LT}=-\pi/2$, circles for $\theta_{LT}=0$ and squares for $\theta_{LT}=\pi/2$. }\label{fig:effetto theta collins ap with GL = 0.2 GT}
\end{figure}




\subsection*{Dihadron asymmetry}

\subsection{Comparison with experimental data}
